Parameter Estimation in Optimal Tolling for Traffic Networks Under the Markovian Traffic Equilibrium

Tolling, or congestion pricing, has emerged as an effective tool for preventing gridlock in traffic systems. However, tolls are currently mostly designed on route-based traffic assignment models (TAM), which may be unrealistic and computationally expensive. Existing approaches also impractically assume that the central tolling authority can access latency function parameters that characterize the time required to traverse each network arc (edge), as well as the entropy parameter $\beta$ that characterizes commuters' stochastic arc-selection decisions on the network. To address these issues, this work formulates an online learning algorithm that simultaneously refines estimates of linear arc latency functions and entropy parameters in an arc-based TAM, while implementing tolls on each arc to induce equilibrium flows that minimize overall congestion on the network. We prove that our algorithm incurs regret upper bounded by $O(\sqrt{T} \ln(T) |\arcsMod| \max\{|\nodesMod| \ln(|\arcsMod|/|\nodesMod|), B \})$, where $T$ denotes the total iteration count, $|\arcsMod|$ and $|\nodesMod|$ denote the total number of arcs and nodes in the network, respectively, and $B$ describes the number of arcs required to construct an estimate of $\beta$ (usually $\ll |I|$). Finally, we present numerical results on simulated traffic networks that validate our theoretical contributions.

==> temp.tex <==
% temp.tex


This work presents a two-timescale discrete-time stochastic dynamical system to describe the joint evolution of,

in which tolls are iteratively modified while 

models travelers as self-interested agents who iteratively adapt their routing strategies

introduces a \textit{marginal cost tolling scheme}

We explain each of these modeling choices below.

==> temp_figures_other.tex <==

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/phi_dynamics.eps}
    \caption{Latency-to-go $\varphi$ vs. time index $n$ for the Condensed DAG in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:phi_dynamics}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/cost.eps}
    \caption{Cost functions for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:cost}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/final_no_toll.eps}
    \caption{No Toll: Steady state MTE flows for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:final_no_toll}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/final_with_toll.eps}
    \caption{With Toll: Steady state MTE flows for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:final_with_toll}
\end{figure}


==> temp_statements_proof_sketches.tex <==


\vspace{1mm}
\begin{proof}(\textbf{Proof Sketch})
The following proof sketch parallels that of \cite{Chiu2023ArcbasedTrafficAssignment}, Lemma 3, and is included for completeness.

Part 1) holds because, with respect to $\mathcal{F}_n$, the only source of stochasticity in $M_a[n+1]$ is ude to the input flows $\eta_{i_a}[n+1]$, which are i.i.d. Part 2) follows from the flow continuity equations in \eqref{Eqn: General Network, w flow, discrete}, which can be used to establish recursive upper bounds on each $\arcLoadModDiscrete_a[n]$ and $\costToGo_a(\arcLoadModDiscrete[n])$, in increasing order of depth and height, respectively (since flows run from origin to destination, and cost-to-go values are calculated in the opposite direction). These bounds can then be used to recursively establish upper and lower bounds for each $\probDist_a[n]$, and consequently each $\arcLoadModDiscrete[n]$, in order of increasing depth. Finally, Part 3) can be proved by establishing that $\rho_a$ is continuously differentiable, with bounded derivatives over the compact domain defined by the bounds on $\arcLoadModDiscrete[n]$ established in the second part of the lemma. 
For details, please see Appendix \ref{subsubsec: A2, Proof of Lemma: Technical Conditions for Stochastic Approximation, 1}.
\end{proof}




\begin{proof}(\textbf{Proof Sketch})
To establish Lipschitz continuity, we prove that the functions listed here are continuously differentiable, with derivatives uniformly bounded over their domains. This in turn can be done by recursively computing their derivatives in increasing order of height or depth. 
For details, please see Appendix \ref{subsubsec: A2, Proof of Lemma: Technical Conditions for Stochastic Approximation, 2}.
\end{proof}
